Adversarial Gradient Driven Exploration for Deep Click-Through Rate Prediction

Exploration-Exploitation (E{\&}E) algorithms are commonly adopted to deal with the feedback-loop issue in large-scale online recommender systems. Most of existing studies believe that high uncertainty can be a good indicator of potential reward, and thus primarily focus on the estimation of model uncertainty. We argue that such an approach overlooks the subsequent effect of exploration on model training. From the perspective of online learning, the adoption of an exploration strategy would also affect the collecting of training data, which further influences model learning. To understand the interaction between exploration and training, we design a Pseudo-Exploration module that simulates the model updating process after a certain item is explored and the corresponding feedback is received. We further show that such a process is equivalent to adding an adversarial perturbation to the model input, and thereby name our proposed approach as an the Adversarial Gradient Driven Exploration (AGE). For production deployment, we propose a dynamic gating unit to pre-determine the utility of an exploration. This enables us to utilize the limited amount of resources for exploration, and avoid wasting pageview resources on ineffective exploration. The effectiveness of AGE was firstly examined through an extensive number of ablation studies on an academic dataset. Meanwhile, AGE has also been deployed to one of the world-leading display advertising platforms, and we observe significant improvements on various top-line evaluation metrics.

==> Latex/Chapters/4-theore.tex <==
\section{Theoretical analysis} \label{sec:Theoretical}

In this section, we prove that the one-step model training update vector is equivalent to the vector with the uncertainty as the step size and the unit adversarial perturbation vector as the direction. In another word, it is to prove the equivalence of Eqn.(\ref{Delta}) and Eqn.(\ref{eq:advs}). It can verify our motivation on adversarial gradient. 

Before Theorem \ref{thm1}, we shall give definition around one-step training update vector and adversarial perturbation, which is shown as Definition \ref{def1}.
\begin{Definition}
\label{def1}
Give sample $\{x,y^*\}$ with CTR $p$, where $x$, $y^* \in\{0,1\}$ is the label and CTR $p$ means label $y^*$ is $1$ with probability $p$ and $0$ with probability $1-p$ and give a prediction CTR model $y'=f(E(x)|\Theta)$ which is the same as Eqn.(\ref{eq:ctr}). The adversarial perturbation with step-size $\lambda$ as $\vec{g}_{adv}(\lambda)$ of sample $\{x,y^*\}$ is defined as 
 \begin{equation}
 \vec{g}_{adv}(\lambda) =\argmax_{\|x_{adv}\|_2\leq \lambda}f(E(x)+x_{adv}|\Theta).
  \end{equation}
  The one-step update training update vector with learning rate $\lambda$ as $\vec{g}_{train}(\lambda,y^*)$ of sample $\{x,y^*\}$ is defined as 
 \begin{equation}
\vec{g}_{train}(\lambda,y^*)=\argmax_{\|x_{train}\|_2\leq \lambda}{\mathcal{L}}(f(E(x)+x_{train}|\Theta),y^*),
  \end{equation}
  where $\mathcal{L}$ is the cross entropy loss.
\end{Definition}

 \begin{Theorem}
 \label{thm1}
Give a sample $\{x,y^*\}$ with CTR $p$, and model in Definition \ref{def1}. Assume the gap of CTR and the prediction CTR satisfies a distribution $(y'-p)\in \kappa(\rho)$. The adversarial perturbation $g_{adv}(\lambda)$ and the expectation of training update vector
$\mathbb{E}_{y^*}(\vec{g}_{train}(\lambda,y^*))$ are in the same direction with scale factor $\rho$.
 \begin{equation}
     \lim_{\lambda \rightarrow 0}( \rho \vec{g}_{adv}(\lambda) - \mathbb{E}_{y^*}(\vec{g}_{train}(\lambda,y^*)))=\vec{0},
 \end{equation}
 where $\rho$ is random variable and satisfies the distribution $ \rho \in \kappa(\rho)$.
 \end{Theorem}
 The proof of Theorem \ref{thm1} is shown in the supplementary materials. 
 The conclusion of Theorem \ref{thm1} illustrate that when the update step-size $\lambda$ is very small, the adversarial perturbation of embedding parameter in model at training phase is just the adversarial disturbance with step-size following the same distribution as the gap between prediction CTR and CTR. i.e. uncertainty of the prediction CTR.


%\begin{Theorem}
%\label{thm2}
% Give a model with two layer network ReLU with two one-dimension inputs $x\in \mathbb{R}^1$ and $y\in \mathbb{R}^1$, where $x$ is learnable parameter like the cold-start item embedding, $y$ is the input sampled from normal distribution $\mathcal{N}(0,1)$ like the user embedding and parameters in model is fix like the stable parameter in CTR model. The 
%$\mathbb{E}(\|x^{t}-x^{*}\|_1)\geq \|\hat{x}^{t}-x^{*}\|_1.$
% \end{Theorem}
 
 %The conclusion in Theorem \ref{thm2} tells us using the adversarial disturbance as the indicator to do sample selection in the training phase shall boost the converge speed of learning.

 %Combining Theorem \ref{thm1} and Theorem \ref{thm2}, it can be determined that using the confrontation gradient as the exploration strength can indeed accelerate the convergence speed of the model.

